Automatic Heap Layout Manipulation for Exploitation

Heap layout manipulation is integral to exploiting heap-based memory corruption vulnerabilities. In this paper we present the first automatic approach to the problem, based on pseudo-random black-box search. Our approach searches for the inputs required to place the source of a heap-based buffer overflow or underflow next to heap-allocated objects that an exploit developer, or automatic exploit generation system, wishes to read or corrupt. We present a framework for benchmarking heap layout manipulation algorithms, and use it to evaluate our approach on several real-world allocators, showing that pseudo-random black box search can be highly effective. We then present SHRIKE, a novel system that can perform automatic heap layout manipulation on the PHP interpreter and can be used in the construction of control-flow hijacking exploits. Starting from PHP's regression tests, SHRIKE discovers fragments of PHP code that interact with the interpreter's heap in useful ways, such as making allocations and deallocations of particular sizes, or allocating objects containing sensitive data, such as pointers. SHRIKE then uses our search algorithm to piece together these fragments into programs, searching for one that achieves a desired heap layout. SHRIKE allows an exploit developer to focus on the higher level concepts in an exploit, and to defer the resolution of heap layout constraints to SHRIKE. We demonstrate this by using SHRIKE in the construction of a control-flow hijacking exploit for the PHP interpreter.

==> sections/bck_conclusion.tex <==
In the context of the exploitation of heap-based overflows and underflows, heap layout optimisation is a significant problem. Inadvertent access to collateral data can lead to an unstable process and render exploits ineffective. Traditionally, this problem is solved manually and requires extensive knowledge of the application under analysis as well as the allocator that it utilises.

In this paper we have defined the heap layout optimisation problem as a distinct task, within the context of automatic exploit generation. To address this problem we have provided a pseudo-random blackbox approach to heap layout manipulation, and shown that it can produce optimal heap layouts in a significant number of the synthetic experiments we have run. In cases where an optimal layout is not achieved this approach can still on average achieve a layout that places the source and destination buffers close to each other with a relatively low amount of collateral data in between.  

We have also described an end-to-end system for heap layout manipulation in the context of the \PHP language interpreter. This system can discover from the tests distributed with \PHP how to utilise \PHP's API to interact with its allocator, as well as automatically discovering how to allocate data structures on the heap which are likely to be interesting from an exploitation point of view. This information is then combined with our search algorithm to synthesise new \PHP programs which manipulate the heap state to ensure that the destination is placed as close as possible to the source. 

In effect, this system converts vulnerability triggers into inputs which utilise these vulnerabilities to corrupt or read specific heap-based data structures, and to the best of our knowledge it is the first such system to do this automatically.   


==> sections/bck_experiments.tex <==
\newtheorem*{nfisflba}{Noise-free Interaction Sequences, Free List Based Allocators}
\nfisflba The evaluation for the noise-free interaction sequences of free-list based allocators can be found in table~\ref{tab:synth_free_list}. We evaluated our algorithm against \dlmalloc and \avrlibc. As can be seen in the results, an optimal layout was achievable in less than 500,000 guesses on all but one problem. The average number of guesses required was 29,269. The single case in which a non-optimal result was achieved is an overflow scenario where the source size is 64 and the destination size is 4096. In this case, the best layout found places the source 80 bytes from the destination. 

\newtheorem*{nisflba}{Noisy Interaction Sequences, Free List Based Allocators}
\nisflba The latter half of table~\ref{tab:synth_free_list} shows the impact of adding noise to the source and destination allocations. Adding a single noisy allocation, with a size equal to the source, results in a halving of the number of optimal results achieved within 500,000 guesses. The average error ranges from .37 to .68, meaning that the search is still able to manipulate the heap layout to a state that result in an acceptable amount of collateral corruption. With four noisy allocations the number of instances for which an optimal result is found drops further still, with the average error increasing to range from 1.25 to 1.95. It is clear that the search is failing to create a sufficient number of holes to capture the noisy allocations in many instances at this point. 

\newtheorem*{nfisstba}{Noise-free Interaction Sequences, Segregated Storage Based Allocators}
\nfisstba Table~\ref{tab:synth_slab} shows the evaluation results for segregated storage based allocators. segregated storage based allocators appear to present more of a challenge for random search, with optimal results being found for 82\% of the noise-free problems. This is to be expected, due to the extra constraints which segregated storage based allocators impose on the positioning of chunks in memory. The average error is 1.13, although it is worth noting that this is significantly increased by poor performance on a small number of problems when the \texttt{python-malloc} starting sequence is used. If these are excluded then the average error is .25.

\newtheorem*{nisssba}{Noisy Interaction Sequences, Segregated Storage Based Allocators}
\nisssba The addition of noise to the source and destination allocations causes a drop in performance down to the same level as found in free-list based allocators. With a single noisy allocation the average error remains below 1 in most cases, but with four noisy allocations the average error is typically above 1, with a worst case of 3.78. 

\subsubsection{Conclusion}


==> sections/heap_allocator_mechanisms.tex <==
Heap allocators are libraries responsible for servicing dynamic requests for memory allocation and typically expose an interface that complies with the ANSI C~\cite{ANSI:c89} specification for the functions \malloc, \free, \realloc and \calloc. As mentioned in section \ref{sec:introduction}, the specification imposes no restrictions on `\emph{the order and contiguity of storage allocated by successive calls}' to these functions. Thus, the developers of an allocator can choose any combination of data structures and algorithms in their implementation to achieve the best results across whatever measure of success they have, be it minimising fragmentation, maximising speed, increasing security, or some other metric entirely. In the following, we discuss the design choices which have the most impact when it comes to manipulating the heap into a desired state, or that are otherwise significant in differentiating allocators.
\textcolor{red}{Thomas: Readers well-versed in these matters can skip to Section 3.?}


%For example, an allocator designed with no goal other than servicing requests as fast as possible might simply record a continuously incrementing pointer as the next return value for \malloc and do nothing on calls to \free. More reasonable trade-offs still result in drastically different data structures and algorithms in use. In this section we elaborate on the differing aspects of heap allocators that are relevant when it comes to optimising a heap layout for exploitation and the experiments that we have performed. The existing literature can be consulted for a thorough taxonomy of allocators~\cite{Wilson:DynamicStorageSurvey95}, in-depth analysis of individual implementations~\cite{Phrack:MaXX, Phrack:AnonFree, Phrack:jp, Phantasmal05Maleficarium, Phrack:ArgpJeMalloc}, and material on trade-offs in allocator design~\cite{DougLeaMalloc, Evans06Jemalloc}.

%The challenge in designing an efficient heap allocator primarily comes from the fact that allocators are \emph{online} algorithms. An allocator must respond to sequences of interactions that are not known upfront and cannot be predicted. Thus, an allocator must be designed to take advantage of regularities in expected frequently occurring interaction sequences, while being resilient against pathological edge cases. As discussed in~\cite{Wilson:DynamicStorageSurvey95}, the approach that a heap allocator takes to memory management can analysed at three different levels of granularity; the general \emph{strategy} for buffer management which the developers wish to encode; an implementable, but high level, algorithm in the form of a \emph{policy} which describes how to manage buffers in compliance with the strategy; the low level \emph{mechanisms} used to actually encode the policy, in the form of the data structures and algorithms that make up the code of the allocator. 

%For example, a strategy aimed at maximising locality of reference might be `\emph{place buffers as close as possible to the last allocated buffer}', which makes the assumption that buffers allocated together are likely to be accessed together. The \emph{next fit} policy is one possible concrete embodiment of this strategy, which starts searching for a free buffer to return at the next address after the last returned buffer. Finally, one could use a linked list ordered by address to store free chunks as the underlying data structure, combined with a linear scan starting from the next highest free buffer after the last returned buffer, as the mechanism which implements the policy. 

%Most modern allocators utilise a combination of approaches to handle memory requests of different sizes. Not all differences in the design choices of an allocator are relevant when it comes to HLM however. 

\subsection{Allocator Policies and Mechanisms}
\subsubsection{Splitting}
Allocators may or may not split blocks of memory to fulfil a request for a smaller block. When blocks are split, the area to use for the allocation may be split from either the beginning or the end of the existing block. 

For example, both \dlmalloc and \avrlibc will split blocks, but the former splits from the front, while the latter splits from the end. If carving takes place from the front then there is space to place another block \emph{after} the returned block, while if carving takes place from the end then there is space to place another block \emph{before} the returned block. In contrast with both of these, \tcmalloc splits only blocks above 32KB in size. 
\textcolor{red}{Thomas: Why the use of `splitting' and `carving'? Isn't all of this splitting?}

\begin{figure}
\centering
\includegraphics[scale=.45]{images/splitting.pdf}
\caption{Splitting a block of size 128 on a request for an allocation of size 32 followed by an allocation of size 16. Allocations can be split from the beginning or the end of free blocks, resulting in two different heap layouts, labelled as `A' and `B'. In outcome `A' the allocation of size 16 ends up after the allocation of size 32 as allocations are split from the start of the free area, while in the outcome labelled `B' the allocation of size 16 ends up before the allocation of size 32 as allocations are split from the end of the free area.}
\label{fig:splitting}
\end{figure}

Figure~\ref{fig:splitting} shows two possible state transitions for the heap state, depending on what form of splitting is used. In the first outcome, labelled `A', the block of size 32 ends up before the block of size 16, while in the second outcome, labelled `B', outcome the order is reversed. This is significant if one requires a particular ordering for the blocks resulting from two allocations.

\subsubsection{Coalescing}
When blocks are freed, and other free blocks are immediately adjacent, they may be coalesced into a single, larger, free block. Allocators may or may not do this, or they may use an intermediate approach where coalescing is delayed, but will eventually happen if some event occurs (such as the number of uncoalesced blocks exceeding a threshold). If immediate coalescing is used (as in modern \dlmalloc and \avrlibc) it is not possible to have two free blocks next to each other since they would immediately be coalesced into a single larger free block. However, if delayed coalescing is used (as in early versions of \dlmalloc and some versions of the \Windows userland~\cite{McDonald09PracticalXPExploitation} and kernel heaps~\cite{Mandt11KernelPoolExploitation}) it is possible to have multiple free chunks adjacent to each other. 

\begin{figure}
\centering
\includegraphics[scale=.45]{images/hole_creation_coalescing.pdf}
\caption{Hole creation via free. The outcome labelled `A' results from an allocator with immediate coalescing, where a hole of size 256 is produced from two frees of size 128. The outcome labelled `B' results from an allocator with delayed coalescing, where two holes of size 128 are produced from two frees of size 128.}
\label{fig:hole_creation_coalescing}
\end{figure}

Figure~\ref{fig:hole_creation_coalescing} shows two possible state transitions for the heap state, depending on what form of coalescing is used. If the goal is creating holes of size 128, the second free is either useful or counterproductive, depending on whether or not delayed coalescing is in use. 

\subsubsection{Fits}
When searching for a suitably sized free block to use for an allocation, the allocator has several options on where to start the search and on what condition to end it. The most common approach is \emph{best-fit} in which a free block with size closest to that of the requested allocation size is guaranteed to be found, split if necessary, and returned. Alternatives include \emph{first fit} and \emph{next fit}. In first fit, the first block encountered during the search that is large enough to fulfil the requested allocation is selected, split if necessary, and returned. In next fit, the next search for a free block continues in the free list from the last index reached by the previous search. \textcolor{red}{Thomas: Can the previous sentence be clarified?} The fit policy in use is relevant to HLM in that it influences which block is selected for a particular size. \textcolor{red}{Thomas: Is
fit policy the best word, or is `search policy' perhaps better? Not sure.}

%For example, assume that there is a single hole of size $x$ and a single hole of size $y$, with $y > x$, and we wish to fill the hole of size $x$. If best fit is in use, then triggering an allocation of size $x$ will fill the hole. However, if first fit is in use then our allocation of size $x$ may be placed in any hole $h$ such that $h \ge x$. If the hole of size $y$ is found by the algorithm before the hole of size $x$ then it will be used to service the request.  

\subsubsection{Segregated Free Lists}
Some allocators, such as \avrlibc, use a single free-list in which all free chunks are stored. While simple to implement, this approach has a significant disadvantage: The
entire list may need to be scanned in order to determine which block is a best-fit
for an allocation. An alternative, as found in modern \dlmalloc, is \emph{segregated free lists}, in which multiple free lists are used. Blocks of similar size are kept in the same list. With segregated free lists one can efficiently check to see if a free block of a particular size exists. For the purposes of HLM, a single free list or multiple free lists do not significantly impact the complexity of the problem, or the approach this paper takes. 

\subsubsection{Segregated Storage}
\label{sec:segregated_storage}
Segregated storage is a mechanism whereby contiguous areas of memory are set aside for the allocation of blocks of a single size. For example, on the first request for a block of size 32 the allocator might obtain one or more pages from the operating system and subdivide those pages into blocks of size 32. The blocks will then not be further split or coalesced.

%These blocks could be inserted into a free list, or more commonly a bitmap is associated with this \emph{run} of pages which indicates which indices are free and which are allocated. Finding a free block now no longer requires traversing a list. Instead the address of a block can be calculated via simple arithmetic over the base address of the run and the index of the block the developer wants the address of. Along with potential speed increases, this also removes the need for the in-band meta-data often used to maintain free lists, resulting in improved memory efficiency and also potentially improving the security of the allocator as in-band meta-data is a popular target in memory corruption exploits.

Whether segregated storage is in use has a significant impact on how one approaches HLM. The impact this single design decision can have on heap layout is highlighted in the contrast between Figure~\ref{fig:sample_dlmalloc} and Figure~\ref{fig:sample_tcmalloc} in the appendix. Both figures show the heap state after an identical series of approximately 100 interactions consisting of allocations of three different sizes and a number of frees. Figure~\ref{fig:sample_dlmalloc} shows \dlmalloc, which does not use segregated storage. 
We can see that allocations of different sizes end up alternating in memory. Figure~\ref{fig:sample_tcmalloc} shows \tcmalloc, an allocator which does use segregated storage, resulting in three distinct memory regions, each of which contains allocations of a single size. 

\subsubsection{Non-Determinism}
While most allocators are deterministic in their operations, some allocators use non-determinism in allocation as part of an effort to make exploitation more difficult. This differs from traditional Address Space Layout Randomisation (ASLR) which randomises the base address of the heap, to prevent an attacker knowing where it is located in memory. Non-determinism in the allocation process works alongside ASLR to add randomisation to the state transitions of the allocator itself. This is problematic for HLM as it means that over multiple runs of a program from the same starting state, the same sequence of interactions may produce a different layout each time. Although not common, this behaviour can be found in at least two mainstream allocators, namely the \WindowsTen
\textcolor{red}{Thomas: Heap block layout randomization was introduced in Win7 IIRC} the Low Fragmentation Heap (LFH)~\cite{Yason16Windows10} and \jemalloc. 

\subsubsection{Treatment of Larger Allocations}

Most allocators use different algorithms and data structures to handle allocations of sizes that they consider to be small versus those they consider to be large. For example, an allocator might use segregated free lists for allocations up to a certain size and simply use \mmap and \munmap to manage allocations above that size. The threshold above which an allocator considers an allocation to be large can varies by allocator, operating system, and architecture on which the allocator is running.

\subsection{Allocators}
\label{sec:allocators}

For experimentation and evaluation we selected several real world allocators, implementing a variety of different strategies and policies. We will refer to \dlmalloc and \avrlibc as \emph{free list based} and \tcmalloc and \PHP as \emph{segregated storage based}. An overview of the allocators selected can be found in the appendices, in Table~\ref{tab:allocator_features}, but their relevant nuances are as follows:

\newtheorem*{avrlibcth}{avrlibc 2.0}
\avrlibcth An allocator aimed at embedded systems~\cite{avrlibc} which uses best fit search over a single free list. The maximum heap size and its location are fixed at compile time. If an existing free chunk of sufficient size does not exist, a new chunk is split from the remaining heap space.

\newtheorem*{dlmallocth}{dlmalloc 2.8.6}
\dlmallocth A general purpose allocator~\cite{DougLeaMalloc} using best fit search over segregated free lists for blocks with size less than 256KB. Free blocks less than 256 bytes in size are organised in linked lists, while those above 256 bytes, but less than 256KB, are kept in tries. Allocation requests for sizes greater than 256KB use \mmap. The \libc allocator, \ptmalloc, is based on \dlmalloc. 

\newtheorem*{tcmallocth}{tcmalloc 2.5.1}
\tcmallocth Intended as a more efficient replacement for \dlmalloc and its derivatives, especially in multithreaded environments~\cite{tcmalloc}. Sizes above 32KB are allocated using best-fit search from a linked-list of free pages, and splitting and coalescing may take place. Segregated storage is used for sizes below 32KB.

%\newtheorem*{jemallocth}{jemalloc 5.0.1}
%\jemallocth A segregated storage based allocator utilised as the system allocator on \FreeBSD, in \Firefox and in a variety of other applications. If all allocations are less than 16KB in size then the allocator behaves deterministically. Allocations above 16KB in size have a random offset added to the base of the page they are placed within which may impact the layout of the heap at addresses above such allocations.

\newtheorem*{phpth}{PHP 7}
\phpth The allocator for version 7 of the \PHP language interpreter. Sizes above 2MB in size are allocated via \mmap. Sizes below 2MB but above 3/4 of the page size are rounded to the nearest multiple of the page size and are allocated on page boundaries using best-fit over a linked list of free pages. Sizes that are less than 3/4 of a page are rounded up to the next largest predefined small size, of which there are 30 (e.g. 8, 16, 24, 32, ..., 3072), and are allocated from runs using segregated storage. 



%In the above do we want a heapviz diagram of the whole heap after a lot of interactions (more impressive but i'm not sure how to embed it) or a custom made drawing of part of the heap after a small number of interactions. 

%Insert example of two diffrent starting states resulting in two different outcomes after a series of allocations
%Define the heap layout optimisation problem formally

%For our purposes we can consider a heap to be represented by a set of tuples $A$ of the form $(a_i, a_j)$, representing ranges of memory that are managed by the allocator and currently considered to be \emph{allocated}, and a second set of tuples $F$ of the form $(f_i, f_j)$, representing ranges of memory that are managed by the allocator and are currently considered to be \emph{free}.  


